Give Me More Details: Improving Fact-Checking with Latent Retrieval

Evidence plays a crucial role in automated fact-checking. When verifying real-world claims, existing fact-checking systems either assume the evidence sentences are given or use the search snippets returned by the search engine. Such methods ignore the challenges of collecting evidence and may not provide sufficient information to verify real-world claims. Aiming at building a better fact-checking system, we propose to incorporate full text from source documents as evidence and introduce two enriched datasets. The first one is a multilingual dataset, while the second one is monolingual (English). We further develop a latent variable model to jointly extract evidence sentences from documents and perform claim verification. Experiments indicate that including source documents can provide sufficient contextual clues even when gold evidence sentences are not annotated. The proposed system is able to achieve significant improvements upon best-reported models under different settings.

==> tables/constraints.tex <==
\begin{table}[t!]
\centering
\caption{Collection of logic factors and its imposed constraint set $\mathcal{Z}_{f}$.}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{ll}
\toprule
Factor Name & Imposed Constraint   \\
\midrule 
\texttt{XOR} &  $\sum z_{k} =1$ \\
\texttt{AtMostOne} & $\sum z_{k} \leq 1$  \\
\texttt{BUDGET}  & $\sum z_{k} \leq B$  \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\label{tab:constraint set}
\vspace{-0.1in}
\end{table}

==> tables/language.tex <==
\begin{table*}
\centering
\scalebox{0.85}{
\begin{tabular}{lccccc}
\toprule
Language & Code & Fact-Checker & Language Family & Number  \\
\midrule
 Arabic & ar &  misbar.com & Afro-Asiatic &1,999 \\
 Bengali & bn & dailyo.in &  IE: Indo-Aryan & 556\\
 Spanish & cs &  chequeado.com &  IE: Romance &1,329 \\
 Persian & fa & factnameh.com & IE: Iranian  & 278\\
 Indonesian & id &  cekfakta.com &  Austronesian &3,440 \\
 Italian & it & pagellapolitica.it &  IE: Romance &1,435 \\
 Hindi & hi & hindi.newschecker.in &  IE: Indo-Aryan & 1,431\\
 Gujarati & gu &  gujarati.newschecker.in &  IE: Indo-Aryan & 125 \\
 Georgian & ka &  factcheck.ge &  Kartvelian & 1,947\\
 Marathi & mr &  marathi.newschecker.in &  IE: Indo-Aryan  & 85\\
 Punjabi & pa & punjabi.newschecker.in.txt &  IE: Indo-Aryan  & 102\\
 Polish & pl &  demagog.org.pl &   IE: Slavic & 1,697\\
 Portuguese & pt & poligrafo.sapo.pt & IE: Romance & 7,554 \\
 Romanian & ro & factual.ro &  IE: Romance & 889\\
 Norwegian & no &  faktisk.no &  IE: Germanic  &399 \\
 Sinhala & si &  srilanka.factcrescendo.com &  IE: Germanic & 80\\
 Serbian & sr &  istinomer.rs & IE: Slavic & 765 \\
 Tamil & ta &  youturn.in &  Dravidian & 1,403\\
 Albanian & sq & kallxo.com &  IE: Albanian & 660 \\
 Russian & ru &  factcheck.kz & IE: Slavic & 434\\
 Turkish & tr &  dogrulukpayi.com & Turkic &1,639 \\
 Azerbaijani & az &  faktyoxla.info &   IE: Romance &247 \\
 German & de &  correctiv.org &   IE: Germanic & 914\\
 Dutch & nl &  nieuwscheckers.nl &   IE: Germanic & 166 \\
 French & fr & fr.africacheck.org &  IE: Romance & 194  \\
\bottomrule
\end{tabular}}
\caption{Coverage per language of the XFact dataset. XFact contains 25 typologically diverse languages across 11 language families. }
\label{tab:language}
\vspace{-6mm}
\end{table*}

==> tables/meta.tex <==
\begin{table}
\centering
\scalebox{0.95}{
\begin{tabular}{l|cc}
\toprule
Extractors & mBERT-Based  & Graph-Based\\
\midrule
Snippets (HardKuma)  & 42.55 & 42.71\\
Snippets (Ours)  & \textbf{43.82}  & \textbf{44.46} \\\cmidrule(lr){1-3} 
Documents (Surface) & 45.23 & 45.43 \\
Documents (Semantic) & 45.88  & 46.12 \\
Documents (Hybrid) & 45.91  & 46.03 \\
Documents (HardKuma) & 47.84  & 48.26\\
Documents (Ours) & \textbf{51.25} &  \textbf{51.66}\\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{Effect of metadata: F1 results on the test set.}
\label{tab:meta}
\vspace{-4mm}
\end{table}


==> tables/new.tex <==
\begin{table}[t]
\centering
\scalebox{1}{
\begin{tabularx}{8cm}{X}
\toprule
\textbf{Claim}: Trump said: ``"In New Hampshire, I spent $3 million. Jeb Bush spent $44 million. He came in five, and I came in number one."''.
\midrule
\textbf{Metadata}: \\
\textbf{Speaker}: Tim Pawlenty; \textbf{Domain}: Politics; \textbf{Date}: 2011/01/11;
\midrule
\textbf{Evidence}: \\
1. There were several single-year decreases in state spending, two during Pawlenty’s tenure as governor (2009 and 2004), \textbf{but also two before he was governor (1986 and 1983)}. \\
2. Pawlenty did reduce spending for the two-year budget cycle for the first time since 1960, but the major reduction in the 2010-2011 budget cycle was achieved with \textbf{a one-time infusion of federal dollars and measures that delayed spending rather then permanently reducing it}.
\midrule
\textbf{Factuality}: Mostly False
\bottomrule
\end{tabularx}}
\vspace{-3em}
\caption{An example of a fact-checked statement and its associated metadata. The evidence shows that there exist the other two single-year decreases in state spending. Also, the reason of the decrease of the two-year budget is different calculation metrics were used (as highlighted). Therefore, the fact-checker gave the verdict \textit{Mostly False}. }
\label{tab:example}
\vspace{-2em}
\end{table}
